Strong Duality in Nonconvex Quadratic Problems with Separable Quadratic Constraints

We study nonconvex quadratic problems (QPs) with quadratic separable constraints, where these constraints can be defined both as inequalities or equalities. We derive sufficient conditions for these types of problems to present the S-property, which ultimately guarantees strong duality between the primal and dual problems of the QP. We study the existence of solutions and propose a novel distributed algorithm to solve the problem optimally when the S-property is satisfied. Finally, we illustrate our theoretical results proving that the robust least squares problem with multiple constraints has the strong duality property.

==> preamble.tex <==
% Packages and environments
% -------------
%\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsopn}
\usepackage{braket}
\usepackage{bm}
\usepackage{algpseudocode}   % [noend]
\usepackage{enumitem}
\usepackage{etoolbox}
\usepackage{hyperref}
\usepackage{algorithm}
\usepackage{braket}                            % Incorporates \set{} notation
\usepackage{doi}                % Support for doi numbers

% TODO NOTES: DELETE AFTER DRAFT IS READY
% Select what to do with todonotes: 
% \usepackage[disable]{todonotes} % notes not showed
\usepackage[disable]{todonotes}   % notes showed "draft"; not showed "disable"

% Fixes journal style when using cleveref (Springer's bug)
\makeatletter \let\cl@chapter\relax \makeatother

% Cleveref with IEEEtrantools
\usepackage[nameinlink,noabbrev,capitalise]{cleveref}     % Order is important   
\usepackage[retainorgcmds]{IEEEtrantools}


% Color definitions
\RequirePackage{xcolor}[2.11]
\colorlet{dark_green}{green!50!black}
\colorlet{dark_red}{red!50!black}

% Hyperref coloring
\hypersetup{
  linktoc=all,                  % Set to all if you want both sections and subsections linked
  colorlinks   = true,          % Colours links instead of ugly boxes
  urlcolor     = dark_red,      % Colour for external hyperlinks    % blue
  linkcolor    = dark_green,    % Colour of internal links    % blue
  citecolor    = dark_red       % Colour of citations    % red
}


% TikZ
% -------------
\usepackage{pgfplots}
\usetikzlibrary{arrows,positioning}
\pgfplotsset{compat=1.5}
\pgfplotsset{plot coordinates/math parser=false}
\pgfplotsset{major grid style={dashed,line width=0.5pt}}


% Environments.
% -------------
%\newsiamremark{assumption}{Assumption}
%\newsiamremark{remark}{Remark}
\spdefaulttheorem{assumption}{Assumption}{\bf}{\it}


% Cref names for user defined environments
% -------------
\crefname{assumption}{Assumption}{Assumptions}
%\crefname{lemma}{Lemma}{Lemmas}
%\crefname{theorem}{Theorem}{Theorems}
%\crefname{proposition}{Proposition}{Propositions}
%\crefname{corollary}{Corollary}{Corollaries}

